Neural Image Re-Exposure

The shutter strategy applied to the photo-shooting process has a significant influence on the quality of the captured photograph. An improper shutter may lead to a blurry image, video discontinuity, or rolling shutter artifact. Existing works try to provide an independent solution for each issue. In this work, we aim to re-expose the captured photo in post-processing to provide a more flexible way of addressing those issues within a unified framework. Specifically, we propose a neural network-based image re-exposure framework. It consists of an encoder for visual latent space construction, a re-exposure module for aggregating information to neural film with a desired shutter strategy, and a decoder for 'developing' neural film into a desired image. To compensate for information confusion and missing frames, event streams, which can capture almost continuous brightness changes, are leveraged in computing visual latent content. Both self-attention layers and cross-attention layers are employed in the re-exposure module to promote interaction between neural film and visual latent content and information aggregation to neural film. The proposed unified image re-exposure framework is evaluated on several shutter-related image recovery tasks and performs favorably against independent state-of-the-art methods.

==> legacy/1_introduction_v1.tex <==

\section{Introduction}

\xinyu{Which term could be used to refer to all these tasks? Frame restoration?}

\begin{figure}  % figure of 3d block
%	teasing figure: a visual latent space, different exposure lead to different images
	\centering
	\includegraphics[width=1.05\columnwidth]{figs/teasing_figure2.pdf}
	\caption{
		In the simulated exposure process, neural films get exposed to portions of visual content from the visual latent space under the control of a neural shutter to generate frames of  target moments with desirable quality. 
		By constructing the visual latent space from real-captured sensor data and performing the simulated shutter-controlled exposing process,
		multiple frame restoration tasks are addressed simultaneously.
		{
		% in which a film takes samples from the optical content under the control of a shutter.
		% This work seeks to find a way to simulate the exposing process with a neural network.
		%Core idea of the proposed method.
		%Video can be viewed as a series of temporal sampling of the optical content.
		%By Simulating this process with a neural network, 
		%we can control the quality of the image through the simulated shutter.
		}
	}
	\label{fig:teasing_figure}
\end{figure}

A video camera is a device for capturing visual content from optical signals over time. 
By means of a series of exposure processes in which a shutter selects portions of visual content to get the film or sensor get exposed, a sequence of frames is produced, reflecting the dynamic appearance of the scene.

\begin{figure*}[h!]
	\centering
	\includegraphics[width=1.0\textwidth]{figs/fig_structure_overview.pdf}
	\caption{Structure overview of the proposed method. By specifying a neural shutter of $\mathcal{T}(t_a, t_b)$, a corresponding target image can be obtained.
	}
	\label{fig:structure_overview}
	\vspace{-1em}
\end{figure*}


% existing methods从issues的成因和特点出发来解决问题
Constrained by the capability of the device, videos commonly suffer from issues including discontinuity, motion blur, rolling shutter effect, etc.
Existing methods tend to address these issues from the perspective of their specific causes and characteristics.
For example, algorithms for frame interpolation~\cite{bibid} typically estimate the motion field of the frames to predict the trajectory of each pixel.
To restore the motion blur, deblurring algorithms~\cite{bibid} may establish the motion model that causes blurring, 
restoring the confused temporal information with an implicitly or explicitly estimated the blurring kernel, 
or collecting information from adjacent frames as an extra clue.
For rolling shutter correction, 
algorithms~\cite{bibid} typically evaluate the velocity of each pixel, then infer and reverse the displacement of them to restore the temporal misalignment.
Although these methods are effective, they are limited to their specialized domains.

% 没有从特定的成因或特性出发，我们着眼于所有图片的共同点——曝光过程。
Instead of delving into specific causes or characteristics, 
we propose to establish a model simulating the process of exposure to restore arbitrary expected frames.
Theoretically, sharp images of arbitrary instants within the shooting period can be obtained through exposure processes, as the optical signals entering the lens carry comprehensive visual content.
If we can reconstruct the visual content of the optical signals into a visual latent space, and devise a structure to simulate the exposure process, we can break the limit of the physical device and get rid of the aforementioned issues. 

To 
The events are a type of data generated by event cameras~\cite{bibid}, 
which encodes the variation of the scene in extremely high temporal resolution with low energy and memory cost.
complementing the information provided by the frames.
By jointly leveraging frames and events, we can construct a comprehensive visual latent space. 

To build a structure simulating this behavior, several requirements must be met. 
Firstly, the film must be able to interact and exchange information with the visual latent space.
Secondly, the visual latent space should be time-aware, 
allowing the neural film to identify the required temporal information. 
Lastly, the structure should be controlled by the neural shutter, ensuring that the exposure results are controllable. 
Building this structure with attention mechanism~\cite{Transformer}~\cite{ViT} is a viable option that fulfills all these requirements.
Specifically, attention operation enables the neural film to exchange information with neural optical content.
And we make the optical content time-aware by incorporating time encodings that describe its temporal structure.
We design the time encodings and neural shutter to serve as positional encodings of neural optical content and neural film respectively,
thereby the neural film can locate and collect information through the attention operation under the control of the neural shutter.
After the attention operation, the neural film has sufficient visual information of the instant specified by the neural shutter.
And similar to an exposed film, an image of specified instant can be developed from it.


By adjusting the neural shutter, we can control the content and quality of the produced images.
% 由于模拟出来的曝光过程不会受到真实相机的性能限制，我们可以将参数调整为理想状况, 进而得到关于任意时刻不包含上述问题的的图像
As the simulated exposure is not restricted by the camera capability,
we can configure the shutter to a series of densely specified instants to produce frames at a high frame rate,
while keeping the images sharp and without distortion by setting the shutter to open and close at a same instant.
In this way, we can generate images meeting the requirements of a variety of video restoration tasks, 
including frame interpolation, deblurring, and rolling shutter correction, as shown in fig.~\ref{fig:teasing_figure}.
When multiple issues impair the given videos, the proposed method can address them simultaneously,
achieving goals like jointly deblurring and frame interpolation, jointly deblurring and rolling shutter correction, etc.
We unify a variety of video restoration tasks into a single framework.

%Event camera is a new type of sensor able to record the dynamic content of the scene in high temporal resolution.
%Each event corresponds to a change in the brightness of a pixel, 
%and provides information about the time, location, and polarity of the change. 
%This allows event cameras to capture high-resolution visual information at the very high temporal resolution, 
%making them particularly useful for capturing fast-moving scenes or dynamic environments. 

% A neural film is a pre-defined feature pyramid that works as the information collector. The neural shutter is a pair of time encoding, indicating the range of visual content that the target image is expected to represent.

%%To organize the components to mimic this behavior, there are two points is required.
%To organize the components to mimic this behavior, 我们需要做到如下几点：
%首先, the information of optical content should be time-aware, 以便于我们能够定位所需的时域信息 % 可寻址 The neural optical content is imbued with time encodings that describe the 
%其次, the structure should be controlled by the neural shutter, 这样曝光的结果才是受控的
%最后, the film should be able to interact and exchange information with the optical content.
%综上所述，The attention mechanism is a good option.
% In an exposure process, the film samples information from the visual latent space under the control of the shutter. 
% The information reaching the film during an open period of the shutter is summarized as a frame.


==> legacy/1_introduction_v3.tex <==

\section{Introduction}

\begin{figure}  % figure of 3d block
%	teasing figure: a visual latent space, different exposure lead to different images
	\centering
	\includegraphics[width=1.05\columnwidth]{figs/teasing_figure2.pdf}
	\caption{
		% In the simulated exposure process, neural films get exposed to portions of visual content from the visual latent space under the control of a neural shutter to generate frames of  target moments with desirable quality. 
		We reconstruct the visual content of the scene into a visual latent space leveraging sensor data including real-captured frames and event streams. 
  % By constructing the visual latent space from real-captured sensor data and performing the simulated shutter-controlled exposing process,
By re-expose the real-captured images with a shutter of desired rate, speed, and manner,		
  multiple frame restoration tasks are addressed simultaneously.
		{
		% in which a film takes samples from the optical content under the control of a shutter.
		% This work seeks to find a way to simulate the exposing process with a neural network.
		%Core idea of the proposed method.
		%Video can be viewed as a series of temporal sampling of the optical content.
		%By Simulating this process with a neural network, 
		%we can control the quality of the image through the simulated shutter.
		}
	}
	\label{fig:teasing_figure}
\end{figure}

\begin{figure*}[h!]
	\centering
	\includegraphics[width=1.0\textwidth]{figs/fig_structure_overview.pdf}
	\caption{Structure overview of the proposed method. By specifying a neural shutter of $\mathcal{T}(t_a, t_b)$, a corresponding target image can be obtained.
	}
	\label{fig:structure_overview}
	\vspace{-1em}
\end{figure*}

When people shoot a photograph with either a film-based camera or a digital camera, the visual content of the scene in front of the camera is recorded on either an analog film or a digital sensor under the control of a shutter. 
An image is then formed by integrating all incoming photons on the film or sensor during the period of exposure. 
In this process, different shutter strategies bring different imaging effects.
When the shutter speed is slow and there are objects moving in the scene, a blurry image will be produced. When the shutter speed is fast but the shutter frequency is low, the fast-moving objects in the video will suffer from stuttering. When a row-by-row readout scheme is adopted in the exposure process, rolling shutter artifacts such as jello effect will appear. 

The shutter strategy applied to the shooting process can not be changed once a photo is taken.
When the captured photo is affected by shutter-related problems, it is typical to employ post-capture image processing techniques for high-quality image restoration.
There has been a mass of methods for blur removal~\cite{DeblurSurvey, DeblurGAN, DeepDeblur}, video frame interpolation~\cite{a-survey-review, SloMo, DAIN}, and rolling shutter correction~\cite{DSUN, JCD}. 
{
% % If this section is too long, this sentence could be commented. (Got it)
% For the deblur task, a sharp image is restored from a blurry one through a neural network model by either estimating motion/blur kernel or directly outputting the final result;
% for the video frame interpolation task, the motion field between given frames to the target timestamp is first estimated and then employed to combine the given frames to predict an interpolated one; for the rolling shutter correction task, motion field of each row is estimated and then leveraged to restore temporal misalignment among rows.
}
%
However, most existing methods deal with the issues separately, with each model only addressing its specialized issue. 
In this work, we would like to explore a way for \textit{flexible re-exposure of a captured photo}.
Similar to refocusing an image captured by a light field camera, the re-exposure method aims at adjusting the shutter (\eg, timing, speed, readout scheme) of a captured image in the post-processing to achieve re-exposure.

% describe our idea by making an analogy with the physical imaging process
Inspired by the physical imaging process of a camera
% where an image is dependent on the visual content of the scene and the applied shutter strategy, 
% we propose to re-expose the captured visual content to produce a new image with a desired shutter state under a network-based framework.
we propose a network-based framework to adjust the shutter effect of the image by performing re-exposure on the captured visual content.

The first step is to project the visual content corresponding to the captured scene into a latent space that serves as the basis of re-exposure. 
To thoroughly obtain the visual content, we incorporate data from the traditional camera and event camera.
Since the traditional camera captures scene content through integration, 
there is much confusion and information missing in the recorded photo. 
Recently popular bio-inspired vision sensors like event camera~\cite{EventCmaera-1, EventCamera-2} and spiking camera~\cite{SpikingCamera-1, SpikingCamera-2} are able to record almost continuous brightness change by firing signal asynchronously, providing an opportunity to correct confusion and make up for the missing information. 
Hence with the help of event cameras or spiking cameras, 
it is possible to approximately reconstruct the whole visual content of the scene in the latent space. 
Then, Similar to the camera shutter whose open period determines the content of the scene being recorded,
the content of the re-exposed photo is determined by the neural shutter under this framework. 
Different from the integration of photons in the physical imaging process, 
the neural imaging process is achieved by aggregating content from a visual latent space.
In a film camera, slight chemical changes proportional to the amount of light are first recorded on a film and are then developed into a photograph.
In the re-exposure framework, a neural film is proposed as the carrier for visual content, which would be `developed' by the decoder into the final desired photo.

\xinyu{Maybe the description of the method is not necessary to be so detailed?} The proposed re-exposure framework consists of three parts, including an encoder for constructing the visual latent space, a re-exposure module, and a decoder for producing the target image. To construct the visual latent space, sensor data including frames and events are processed by the encoder, producing the multi-level visual latent space. Then, an attention-based module performs the image re-exposure, in which a neural film is defined to aggregate the content from the visual latent space under the control of a neural shutter. 
Finally, a U-Net like decoder `develops' the exposed neural film into the target image, whose exposure has been adjusted to the desired state. 

% 
\xinyu{Maybe the description of the method is not necessary to be so detailed?}
Specifically, the proposed neural network based re-exposure framework consists of XX modules.
The visual content corresponding to the captured scene is projected into visual latent space by two encoders, \ie, event encoder and frame encoder. Event stream in the desired interval is first represented by voxel grids with several bins and is then fed to a bi-directional recurrent neural network to model brightness change into a sequence of feature pyramids. Frame is encoded by a multi-scale CNN module into a feature pyramid. The concatenation of event encoded feature maps and frame encoded feature maps construct the visual latent space. 
The exposing module(\xu{may be changed to re-exposure module later}) is composed of several self-attention layers and cross-attention layers. 
It takes as input representation in visual latent space, neural film, and positional encodings of both source image and target image and output an exposed film. 
The neural film is a feature pyramid whose elements are learnable parameters and works as an information aggregator.
Event encoded feature maps, frame encoded feature maps and neural film are all divided into non-overlapping windows of the same size similar to SwinTransformer~\cite{}.
Each position in a window has a token and all attention operations are computed over tokens within each window.
Positional encodings corresponding to the desired image are pairs of time encodings used as neural shutter to control the re-exposure process and those corresponding to the source frame(s) are used to provide extra information for the re-exposure process. 
The exposed\xu{re-exposed?} neural film encodes the scene that is desired to be visualized.
Afterwards, a U-Net like decoder is adopted to `develop' the neural film to the desired image.

The proposed neural re-exposure framework provides a novel perspective to unify shutter related image recovery tasks, and is validated on several of them, including image deblur, video frame interpolation , and rolling shutter correction and combination of them. The proposed method, with a unified framework, is able to re-expose different kinds of input image(s) into a desired one by adjusting the neural shutter, as shown in Fig.~\ref{fig:teasing_figure}.


==> legacy/3_problem_v1.tex <==

\section{Problem Analysis}
\label{sec:Problem Setting}
\xinyu{Is it possible to convert this section to an introduction?}

\begin{figure*}
	\centering
	\includegraphics[width=1.0\textwidth]{figs/fig_optical_content_reconstruction.pdf}
	\caption{(a) Illustrates the reconstruction of visual latent space with events and real-captured frame(s). (b) gives a brief illustration of the exposing simulation.}
	\label{fig:visual_latent_space_construction}
	\vspace{-1.0em}
\end{figure*}

%In this section, we mathematically explain the way of obtaining desired images by simulating the exposing process.

When a camera shoots, the visual content of the optical signals that reach the film during the open period of the shutter is summarized as a frame in the exposing process,
which can be represented as:
\begin{equation}
I(x, y; t_{a}, t_{b}) = \frac{1}{T} \int_{0}^{T} \Omega(x,y;t)S_{xy}(t; t_{a}, t_{b}) dt
\label{equ:shutter_operation}
\end{equation}
Here, $\Omega(x,y;t) \in \mathbb{R}^3$ is a mapping from the spatial-temporal domain to the sRGB color space, 
representing the whole of visual content entering the lens within the duration $T$.
$I(x, y; t_{a}, t_{b})$ denotes a pixel at location $(x, y)$, 
whose exposure starts at $t_a$ and stops at $t_b$.
$S_{xy}(t)$ is the function describing the shutter states corresponding to the pixel,
which is defined as 
\begin{equation}
S_{xy}(t; t_{a}, t_{b}) = 
\begin{cases}
0, & t < t_{a} \\
1, & t_{a} \le t < t_{b} \\
0, & t \ge t_{b}
\end{cases}
\label{equ:shutter_func}
\end{equation}
The subscript $xy$ indicates that the shutter function is for the pixel at (x, y) which may vary among locations (e.g. pixels at different scanlines of a rolling shutter image).
Omitting the subscript, $S(t)$ represents a set of shutter functions traversing all pixels, describing the shutter of an image.

According to equ.~\ref{equ:shutter_operation}, we can obtain any image given the $\Omega$ and $S$.
However, real-captured images commonly suffer from the following issues.
The first is discontinuity.
According to equ.~\ref{equ:shutter_operation}, only the information within an interval of $[t_{a}, t_{b}]$ can be recorded.
If the shutter is of a low frequency, the resulting video will appear choppy or jerky.
Another issue is motion blur.
As the pixels are derived by averaging $\Omega(x,y;t)$ over the period of exposure, 
the detailed variation of the optical signals becomes indiscernible, 
resulting in motion blur in the images. 
Additionally, the widely used rolling shutter cameras result in spatial-varying $S(t)$, causing tilting and distortion when the camera or scene is moving.

It can be observed that all these issues are related to the shutter mechanisms, 
implying us to address them with a proper shutter function. 
Although equ.~\ref{equ:shutter_operation} is derived from real cameras with limited capability,
we can extend it to describe an ideal image by conceiving the exposing process of a sensor whose shutter opens and closes at the same instant $t$:
\begin{equation}
I_t(x, y) = \lim\limits_{\substack{t_{a} \to t \\ t_{b} \to t}}  I(x, y; t_{a}, t_{b}) 
\label{equ:target_frame}
\end{equation}
For the image $I_t$, all pixels reflect the visual content of the instant $t$, without motion blur and rolling shutter effect.
And $t$ can be specified to any instant, leading to very flexible frame restoration.

Unfortunately, the conceived sensor does not exist in reality,
and video cameras with extraordinary capabilities are typically very expensive while requiring significant energy and storage.
As a result, it is very difficult to directly capture ideal images with a physical camera.
To this end, we propose to simulate the photographic exposure process with a neural network.
Specifically, we reconstruct the visual content of optical signals $\Omega$ as a latent space, which is termed as visual latent space in this work.
And we design a module where a neural film collects information under the control of a neural shutter.
By setting the neural shutter opening and closing at the same specified instant $t$,
the produced image will be an ideal image of $t$. 
Furthermore, we can obtain any desired image at will by varying the specified instant $t$.

A remaining problem is how to get enough information from the sensor to construct a comprehensive visual latent space.
As a method for restoring the frames, we presume the available real-captured images are of low-frame rate and susceptible to motion blur and distortion,
so that constructing the visual latent space from them is difficult and not reliable.
To complement the real-captured images, we incorporate the data of an event camera, a novel type of neuromorphic vision sensor.
Different from conventional visual sensors, 
event cameras asynchronously capture and record the variation of optical signals in an extremely high temporal resolution (up to $10^{-6}$ second).
Within the filming duration $[0, T]$, we can collect a stream of event data:
\begin{equation}
E=\left\{ e_i \mid e_{i} = (x_i, y_i, t_i, p_i), t_i \in [0, T]   \right\} \\
\label{equ:event_cloud}
\end{equation}
which spread across the whole spatial-temporal domain, complementing the vacant part left by the captured images, as is shown in fig.~\ref{fig:sensor_data}.
Overall, the events capture the dynamics while the frames capture the color and texture.
By leveraging the information from both sensors, 
we can get sufficient information to comprehensively construct the visual latent space. 

To sum up, analogous to a physical camera producing photos through shutter-controlled exposing,
we can obtain desired images through a neural simulated exposing process.
Through the parameters of the simulated shutter, we can control the content and quality of produced images at will.



==> legacy/3_problem_v2.tex <==

\section{Problem Setting}
\label{sec:Problem Setting}

\begin{figure*}
	\centering
	\includegraphics[width=1.0\textwidth]{figs/fig_optical_content_reconstruction.pdf}
	\caption{(a) Illustrates the reconstruction of visual latent space with events and real-captured frame(s). (b) gives a brief illustration of the exposing simulation.}
	\label{fig:visual_latent_space_construction}
	\vspace{-1.0em}
\end{figure*}

%In this section, we mathematically explain the way of obtaining desired images by simulating the exposing process.

In camera imaging process, the content of an image is determined by both the scene and the applied shutter during exposure period:
\begin{equation}
I(x, y; t_{a}, t_{b}) = \frac{1}{T} \int_{0}^{T} \Omega(x,y;t)S_{xy}(t; t_{a}, t_{b}) dt
\label{equ:shutter_operation}
\end{equation}
Where, $\Omega(x,y;t) \in \mathbb{R}^3$ represents the visual content of the scene in a duration of $T$. %is a mapping from the spatial-temporal domain to the sRGB color space,  
$I(x, y; t_{a}, t_{b})$ denotes captured image, in which the pixel at (x, y) has an exposure starting at $t_a$ and stopping at $t_b$, and the pixel-wise shutter state is represented by a shutter function  $S_{xy}(t; t_{a}, t_{b}) = sgn(t-t_a) - sgn(t-t_b)$ where $t_a < t_b$

{
% $x \in [0, W], y \in [0, H]$ are the coordinates of the pixels, and $(H, W)$ is the size of the image.
% \begin{equation}
% S_{xy}(t; t_{a}, t_{b}) = 
% \begin{cases}
% 0, & t < t_{a} \\
% 1, & t_{a} \le t < t_{b} \\
% 0, & t \ge t_{b}
% \end{cases}
% \label{equ:shutter_func}
% \end{equation}
% The shutter function set $S=\{S_{xy} | x \in [0, W], y \in [0, H] \}$  determines the content of an image.

% In practical photography, real-captured videos commonly suffer from issues like discontinuity, motion blur, and rolling shutter distortion.
% Based on equ.~\ref{equ:shutter_operation}, we can represent frames with arbitrary issues or without these issues.
}

For an image shot by a rolling shutter camera, $S_{xy}$ for pixels in different rows has different $t_a$ and $t_b$, while the pixels of  a global shutter image share the same $S_{xy}$ for all locations.
For each pixel, whether produced by a rolling shutter or a global shutter, the amount of motion blur can be represented by the value of $\Delta{t} = t_b - t_a$. The larger the value of $\Delta{t}$, the heavier the motion blur.
In addition, with different timing $t_a$ for $S_{xy}$, the image of different moment can be obtained.
In a word, given the visual content $\Omega$, we can represent images produced with the shutter of different manners, speeds, and timings.

However, once an image is captured, the shutter strategy of it can not be changed.
To re-expose the real-captured images to a desired state, our proposed method construct visual latent space based on the frames and events to represent $\Omega$. And we simulate the shutter $S_{xy}$ with a neural shutter, by which we adjust the speed, timing, and manner of the shutter strategy of the image to re-expose the captured image.
Specifically, by constructing the visual latent space from a rolling shutter image and corresponding events, we can specify a neural shutter corresponding to the shutter function of an global shutter image.
When the image is blurry, we can obtain a sharp image by specifying the neural shutter with $t_a=t_b$, achieving the goal of image deblurring.
When a pair of low-frame-rate key frames is given, we can evenly specify a series of neural shutter in between the two frames, producing a video clip of a much higher frame rate.
Furthermore,  the combination of above tasks can be also addressed in a unified way.


% % A remaining problem is how to get enough information from the sensor to construct a comprehensive visual latent space.
% As a method for restoring the frames, we presume the available real-captured images are of low frame rate and susceptible to motion blur and distortion,
% so that constructing the visual latent space from them is difficult and not reliable.
% To complement the real-captured images, we incorporate the data of an event camera, a novel type of neuromorphic vision sensor.
% Different from conventional visual sensors, 
% event cameras asynchronously capture and record the variation of optical signals in an extremely high temporal resolution (up to $10^{-6}$ second).
% Within the filming duration $[0, T]$, we can collect a stream of event data:
% \begin{equation}
% E=\left\{ e_i \mid e_{i} = (x_i, y_i, t_i, p_i), t_i \in [0, T]   \right\} \\
% \label{equ:event_cloud}
% \end{equation}
% which spread across the whole spatial-temporal domain, complementing the vacant part left by the captured images, as is shown in fig.~\ref{fig:sensor_data}.
% Overall, the events capture the dynamics while the frames capture the color and texture.
% By leveraging the information from both sensors, 
% we can get sufficient information to comprehensively construct the visual latent space. 

% Particularly, by conceiving an exposure process whose shutter opens and closes at the same instant $t$, we can obtain a sharp global shutter image:
% \begin{equation}
% I_t(x, y) = \lim\limits_{\substack{t_{a} \to t \\ t_{b} \to t}}  I(x, y; t_{a}, t_{b}) 
% \label{equ:target_frame}
% \end{equation}
% For the image $I_t$, all pixels reflect the visual content of the instant $t$, without motion blur and rolling shutter effect.
% And $t$ can be specified to any instant, leading to very flexible frame restoration.

% \xinyu{TODO: introduce the establish of $\Omega$}
% \xinyu{TODO: introduce the setting of different tasks}

% % The first is discontinuity,  motion blur,
% % According to equ.~\ref{equ:shutter_operation}, only the information within an interval of $[t_{a}, t_{b}]$ can be recorded.
% % If the shutter is of a low frequency, the resulting video will appear choppy or jerky.
% % Another issue is motion blur.
% % As the pixels are derived by averaging $\Omega(x,y;t)$ over the period of exposure, 
% % the detailed variation of the optical signals becomes indiscernible, 
% % resulting in motion blur in the images. 
% % Additionally, the widely used rolling shutter cameras result in spatial-varying $S(t)$, causing tilting and distortion when the camera or scene is moving.

% It can be observed that all these issues are related to the shutter mechanisms, 
% implying us to address them with a proper shutter function. 
% Although equ.~\ref{equ:shutter_operation} is derived from real cameras with limited capability,
% we can extend it to describe an ideal image by conceiving the exposing process of a sensor whose shutter opens and closes at the same instant $t$:
% \begin{equation}
% I_t(x, y) = \lim\limits_{\substack{t_{a} \to t \\ t_{b} \to t}}  I(x, y; t_{a}, t_{b}) 
% \label{equ:target_frame}
% \end{equation}
% For the image $I_t$, all pixels reflect the visual content of the instant $t$, without motion blur and rolling shutter effect.
% And $t$ can be specified to any instant, leading to very flexible frame restoration.

% Unfortunately, the conceived sensor does not exist in reality,
% and video cameras with extraordinary capabilities are typically very expensive while requiring significant energy and storage.
% As a result, it is very difficult to directly capture ideal images with a physical camera.
% To this end, we propose to simulate the photographic exposure process with a neural network.
% Specifically, we reconstruct the visual content of optical signals $\Omega$ as a latent space, which is termed as visual latent space in this work.
% And we design a module where a neural film collects information under the control of a neural shutter.
% By setting the neural shutter opening and closing at the same specified instant $t$,
% the produced image will be an ideal image of $t$. 
% Furthermore, we can obtain any desired image at will by varying the specified instant $t$.

% To sum up, analogous to a physical camera producing photos through shutter-controlled exposing,
% we can obtain desired images through a neural simulated exposing process.
% Through the parameters of the simulated shutter, we can control the content and quality of produced images at will.



==> legacy/4_method_v1.tex <==

\section{Method}

In this section, we present SimXpo, 
a practical approach for \textbf{Sim}ulating the e\textbf{Xpo}sing process.

As shown in fig.~\ref{fig:structure_overview}, the proposed method roughly involves 
construction of visual latent space, exposing simulation, 
and ``developing" target image from the exposed neural film.

\subsection{Construction of Visual Latent Space}
\label{sec:Construction of Visual Latent Space}

\begin{figure*}[h!]
\centering
\includegraphics[width=1.0\textwidth]{figs/fig_exposure_module.pdf}
\caption{Illustration of the exposing simulation. 
(a) illustrates the overall architecture of the exposing module.  
% 	(b) shows the way $\beta^{e}$, $\beta^{f}$, and $\beta^{s}$ are applied to event tokens, frame tokens, and film tokens respectively, which makes the tokens time-aware. 
% \xinyu{TODO: leave out (c), formulate (b) as a moudle}
% In (c), we show the temporal range covered by different instances on the left, and present the timestamps of the instance cross-sections as maps of timestamps on the right, illustrating the way $\beta^{e}$, $\beta^{f}$, and $\beta^{s}$ are generated. 
% The internal structure of the multi-head attention is available in the supplementary material.
}
\label{fig:exposing_simulation}
\vspace{-1.0em}
\end{figure*}

The source from which we construct the visual latent space is the sensor data from synchronized event and conventional cameras.

% events: dynamic aspect
Different from images that are naturally represented as tensors, 
events are a set of quadruples without tensor-like structures.
To process events with convolution networks, 
we need to convert the events into tensors while preserving the information of them.
As shown in fig.~\ref{fig:visual_latent_space_construction}, we use the widely adopted spatial-temporal voxel grid~\cite{voxel_grid} as the representation of events.
The whole events set $E$ are evenly split into $M$ groups according to their timestamps:
\begin{equation}
\resizebox{0.9\columnwidth}{!}{$E_m = \left\{ e_i \mid e_{i} = (x_i, y_i, t_i, p_i), t_i \in [\frac{(m-1)T}{M}, \frac{mT}{M}], \right\}$}
\end{equation}
where $m=1,2, \dots, M$.
Then, we convert each event group $E_m$ into a $B$-channel voxel grid:
\begin{equation}
V_m\left(x, y, t_{b}\right)=\sum_{\begin{array}{c}
	x_{i}=x \atop y_{i}=y
	\end{array}} p_{i} \max \left(0,1-\left|t_{b}-t_{i}^{*}\right|\right)
\end{equation}
where $t_{i}^{*}=\frac{(B-1)\left(t_{i}-t_{1}\right)}{T/M}$ is the normalized timestamp, 
and $t_{b}\in\{0,1,2,...,B-1\}$ is the integer timestamp. % $p_{i}\in\{-1, +1\}$ is the event polarity, 
We sequentially fed $\{V_m\}^{M}_{m=1}$ into a Bi-LSTM network, generating a sequence of $M$ feature pyramids $\mathcal{E}=\{\mathcal{E}_m\}^{M}_{m=1}$, where $\mathcal{E}_m=\{ \mathcal{E}^l_m \}_{l=1}^{L}$, $\mathcal{E}^l_m \in \mathbb{R}^{C_l\times\frac{H}{2^l}\times\frac{W}{2^l}}$, $L$ is the total number of levels, and $C_l$ is number of channels of the $l$-th level.
The detailed structure of the Bi-LSTM encoder is included in the supplementary material.

%frames: static aspect
Aside from $M$ groups of events, 
$N$ frames captured by a conventional video camera are processed by a fully convolutional encoder (e.g. first three stages of ResNet-34~\cite{ResNet}),
producing $N$ feature pyramids $\mathcal{I}=\{ \mathcal{I}_n \}^{N}_{n=1}$, where $\mathcal{I}_n=\{ \mathcal{I}^l_n \}_{l=1}^{L}$, 
$\mathcal{I}^l_n \in \mathbb{R}^{C_l\times\frac{H}{2^l}\times\frac{W}{2^l}}$, $L$ and $C_l$ share the same value as those of $\mathcal{E}$.
% $L$ is the same number of levels as the event feature pyramid, and $C_l$ is the same number of channels of the $l$-th level
Here, $N$ is the available real-captured frames depending on the requirements of tasks.
For example, $N$=1 when a blurry frame is given for deblurring, 
and $N$=2 when two key frames are given for intermediate frame interpolation.
The whole $M+N$ feature pyramids compose the visual latent space. 
$M$ and $N$ can be set without restriction except for the demand of the tasks and the memory cost,
which makes SimXpo compatible with various input settings.


\subsection{Exposure Simulation}

The exposure simulation is performed with an attention-based exposing module. 
In the simulated exposure process, 
the visual latent space and neural film are treated as tokens.
Time-aware attention operations are performed on the tokens,
transferring the expected information to the neural film to get it ``exposed".

%\vspace{-1.0em}
\paragraph{Neural Film} 
A neural film is a pre-defined feature pyramid $\mathcal{X}_i=\{ \mathcal{X}^l_i \}^L_{l=1}$,
where $\mathcal{X}^l_i \in \mathbb{R}^{C_l\times\frac{H}{2^l}\times\frac{W}{2^l}}$, $L$ and $C_l$ share the same value as those of $\mathcal{E}$ and $\mathcal{I}$. 
For each level $\mathcal{X}^l_i$, the neural film is initialized by replicating a learnable embedding $\mathbf{v}^l \in \mathbb{R}^{C_l \times 1 \times 1}$among all locations.
The neural film is designed for collecting information from the visual latent space.
It is worth noting that we can perform exposure simulation multiple times with one neural film loaded at a time, or we can load multiple neural films simultaneously for exposure simulation. Both strategies achieve the goal of producing multiple images, while the former saves memory and the latter is more efficient.
Considering most tasks require only one image at a time, and the memory cost is unbearable when too many neural films are loaded, we load only one neural film $\mathcal{X}_1$ at a time by default in our experiments. 

% As shown in fig.~\ref{fig:exposing_simulation}(a), % each level of the neural film is treated equally with the features of visual latent space at the same level.
% the neural film is divided into sub-windows together with the visual latent space, 
% and the feature points are termed as film tokens.
% Through the exposure simulation, the film tokens collect information about the target frame from the visual latent space,
% resulting in the exposed neural film that is then decoded into the target frame by the decoder.

%The neural film is treated equally to the elements of the visual latent space, guaranteeing the semantic level  
%which implicitly encourages the exposed neural film to share the same semantic level with the frame feature, benefiting the generation of the target image.

\paragraph{Time-aware Attention} 
\xinyu{The equations remain to be checked}
The time-aware attention is the building block of the exposing module.
Different from standard attention operation, we design a series of time encodings 
compatible with different types of sensor data while supporting a manually specifying manner that simulates the behavior of the shutter.

In the attention operation, feature points are treated as tokens.   
Each token in the visual latent space contains a portion of the visual content of a specific range of time.
And the film tokens are expected to collect the visual content about a specified range of time.
To identify the temporal range a token represents or is expected to represent, 
we allocate a time encoding to each of them with a module referred to as a timer.

To represent a timestamp, the following encoding is used:
\begin{equation}
% what does the time encoding looks like
\resizebox{0.9\columnwidth}{!}{
    $\gamma(t)=\left(\sin \left(2^0 \pi t\right), \cos \left(2^0 \pi t\right), \cdots, \sin \left(2^{L-1} \pi t\right), \cos \left(2^{L-1} \pi t\right)\right)$
}
\label{equ:time_encoding}
\end{equation}
In practice, we normalize the whole time span of the sensor data to $[0, 1]$, thus $t$ is a normalized timestamp in $[0, 1]$.
A temporal range is determined by two timestamps $t_a$ and $t_b$. 
Consequently, a temporal range is encoded as:
\begin{equation}
	\mathcal{T}(t_a, t_b) = [\gamma(t_a), \gamma(t_b)]
	\label{equ:time_encoding_pair}
\end{equation}
For frame tokens, event tokens, and film tokes, $t_a$ and $t_b$ are determined in different ways. 

For a frame token, $t_a$ and $t_b$ represent the starting and ending instants of the exposure by which the corresponding frame patch is captured.
When $t_a=t_b$, the token represents a patch from a sharp image (e.g. a key frame for VFI).
When $t_a<t_b$, the token represents a patch from blurry image (e.g. a image for deblurring or joint deblurring and frame interpolation).
When tokes represent patches from RS frame, $t_a$ and $t_b$ of them will vary with the center location of the patches.\footnote{Within an RS patch, the timestamps vary across lines, thus we take the $t_a$ and $t_b$ from the center of the patch.}.

For event tokens, 
we have $t_a<t_b$, and $t_b-t_a$ indicates the time span of the events group.
As the event is grouped evenly, the time span of different group are identical.
And event tokens origin from the same event group share the same $t_a$ and $t_b$.

For film tokes, we manually specify a pair $t_a$ and $t_b$ for each of them, indicates the range of visual content the film token is expected to represent.
We can specify $t_a$ and $t_b$ to values where $t_a \leq t_b$. In particular, we 
can set $t_a=t_b=t$ for all film tokens, and the corresponding target image will be sharp without rolling shutter distortion.
As the time encodings for the film tokens determine the content and quality of the target image, playing the role of a shutter in photography, 
thus we term it as neural shutter. 

With a unified time encoding system. the differences between different types of real-captured images and difference of the requirements of different tasks are reflected by the time encodings,
making the proposed method process them in a unified way.
In the proposed model, the module for generating and allocating time encoding is called a timer.


Based on the time encoding system, we perform the level-wise time-aware attention operation. 
For the $l$-th level, we have $M$+$N$+1 feature maps
$\{ \mathcal{E}^{l}_1, \mathcal{E}^{l}_2, \dots , \mathcal{E}^{l}_M, \mathcal{I}^{l}_1, ... \mathcal{I}^{l}_N, \mathcal{X}^{l}_1 \}$, 
we spatially divide them into $r \times r$ non-overlapped sub-windows, in which each feature point is treated as a token. Consequently, there are $(M+N+1) \times r^2$ tokens for an attention operation, denoted as
$Z = [Z^{\mathcal{E}}, Z^{\mathcal{I}}, Z^{\mathcal{X}}]^T= [ z_1^{\mathcal{E}}, z_2^{\mathcal{E}}, \dots , z_{M \times r^2}^{\mathcal{E}}, z_1^{\mathcal{I}}, z_2^{\mathcal{I}}, \dots, z_{N \times r^2 }^{\mathcal{I}}, z_1^{\mathcal{X}}, z_2^{\mathcal{X}}, \dots, z_{r^2}^{\mathcal{X}} ]^T$
where $Z \in \mathbb{R}^{C^l \times (M+N+1)}$ is a matrix each row of which is a token, $z_i^{\mathcal{E}}$,  $z_j^{\mathcal{I}}$, $z_k^{\mathcal{X}}$ denotes the $i$-th event token, $j$-th frame token, $k$-th film token respectively.

In the self-attention, the tokens are projected to $d$-dimension with three projection layers $f_Q$, $f_K$, and $f_V$, producing query, key, and value matrices $Q$, $K$, and $V$. 
Then the time encoding corresponding to each token is applied to the $Q$ and $K$, producing time-aware query and key matrices $\widetilde{Q}$ and $\widetilde{K}$:  
\begin{equation}
\begin{split}
&[Q, K, V] = [f_Q(Z), f_K(Z), f_V(Z)] \\
&\widetilde{Q}=Q + \mathcal{T}, \widetilde{K}=V + \mathcal{T} \\
&Attention(\widetilde{Q}, \widetilde{K}, V) = softmax(\widetilde{Q}\widetilde{K}^T/\sqrt{d})V    
\end{split}
\label{equ:attention}
\end{equation}
where the tokens exchange information with each other.
In the cross-attention, the operation is almost the same, except that 
\begin{equation}
\resizebox{0.85\columnwidth}{!}{
$[Q, K, V] = [f_Q(Z^{\mathcal{X}}), f_K([Z^{\mathcal{E}}, Z^{\mathcal{I}}]), f_V([Z^{\mathcal{E}}, Z^{\mathcal{I}}])]$
}
\end{equation}
thus the information is transferred from frame tokens and event tokens to the film tokes.
Finally, the film tokens are reshaped back to the feature map, producing the pyramid of exposed neural film $\mathcal{Y}=\{ \mathcal{Y}^{l} \}_{l=1}^L$, where $L$ is the total number of levels. 



% In the following attention-based neural exposure module, $\beta^{f}$ or $\beta^{e}$ act as positional encodings\footnote{In a transformer, the attention operation works with positional encodings that identify the relationship of different tokens} for their corresponding tokens, 
% which will be introduced later.

% 为了模拟快门在摄影中的行为

% Similar to the ,
% the neural shutter determines the content of the target image.
% As shown in equ.~\ref{equ:shutter_func}, two instants $t_a$ and $t_b$ determine a shutter.
% we devise the \textit{neural shutter} $\beta^{s}(t_a, t_b)$,
% where $t_a$ and $t_b$ are manually specified.
% Similar to $\beta^{f}$ and $\beta^{e}$, neural shutters serve as the positional encodings for the film tokens,
% indicating the expected sampling range of the neural optical content for producing an image.
% As previously discussed, the shutter determines the content and quality of images. 
% By adjusting the neural shutter, we can obtain images of desired quality at any specified instant.



%\vspace{-1.0em}
\paragraph{Exposing Module} 
Based on the time-ware attention operations, the exposing module is established.
Specifically, the exposing module is composed of stacked interaction layers performing time-aware self-attention, followed by a summary layer performing time-aware cross-attention, as is shown in fig.~\ref{fig:exposing_simulation}(a).
Additionally, there are structures in between the attention operations for enlarging the receptive field, which are termed as inter-attention layers.
As shown in fig.~\ref{fig:exposing_simulation}(b), the tokens of higher level is upsampled and added to the lower level, and the lower level is processed by a layer of deformable convolution before they are fed into the next attention operation.
% More details of the attention operations are available in the supplementary material.

\begin{figure*}[h!]
	% 使用duration不为0的neural shutter，获取blurry image观察效果
	\centering
	\includegraphics[width=1.0\textwidth]{figs/qualitative.pdf}
	\caption{
		Qualitative results of the simulated shutter-controlled exposure.
		The quality and content of the frames are controlled by the neural shutter.
		% More qualitative results are available in the supplementary material.
	}
	\label{fig:qualitative_results}
	\vspace{-1.0em}
\end{figure*}


% TODO: perform self-supervised training - convert the predicted high-quality image back to the original low-quality ones.
% TODO: use the neural film to transfer the information of last frame into next frame - 比如用于预测光流，比如用于MOT. The neural film of last frame carring previous information. 

\subsection{Decoder}
\label{sec:Decoder}
Similar to the last step of photography where an image is developed from the exposed film,
the decoder ``develop" the target image from the exposed neural film.

The decoder is essentially a U-Net~\cite{U-Net} decoder, which is a widely adopted architecture in generative tasks.
%Although our proposed method do not have a conventional U-Net encoder,
%we find the input of a U-Net decoder can be viewed as a pyramid of feature, which is compatible with our method.
We iteratively feed the pyramid of exposed neural film $\mathcal{Y}^{l}$ 
to the decoder from the coarsest level to the finest level.
Each level is processed by the convolution layers followed by an upsampling layer,
and the upsampled feature is added to a finer level which will be further processed in the next stage.
Finally, the last layer output the target image corresponding to the visual content specified by the neural shutter.
% A detailed description of the neural developer is included in the supplementary material.

\subsection{Versatility}

So far, we have discussed how to obtain favorable images of given instants by simulating the exposure process. 
It is natural to find that many frame restoration tasks can be handled by this approach. 

As shown in fig.~\ref{fig:teasing_figure}, 
many tasks can be viewed as extracting images of specific instants from visual latent space. 
Meanwhile, the proposed method is very scalable and flexible. It is able to construct visual latent space based on sensor data of various settings, and support an arbitrarily specified neural shutter. 
Therefore, our proposed method is competent for various frame restoration tasks,
including deblurring, frame interpolation, and rolling shutter correction.
Furthermore, SimXpo is able to address multiple issues simultaneously, e.g. joint deblurring and rolling shutter correction, joint deblurring and frame interpolation, etc., 
which typically require cascading multiple algorithms.


==> legacy/5_experiment_v1.tex <==

\section{Experiments}

We conduct experiments on multiple shutter-related tasks including deblurring, video frame interpolation (VFI), rolling shutter correction, and jointly deblurring and frame interpolation,
which are tasks with available benchmarks.

\subsection{Training Strategies}

There are two strategies we can adopt for training our model.
The first one is the task-specialized strategy, in which we only train the model to perform the specific task, e.g only providing blurry images only forcing the model to predict the sharp image at the mid instant of the exposure to train a model specialized in deblurring.  
%in accordance with the corresponding rules for a fair comparison.
The second one is the multi-task strategy, in which we randomly feed input of different tasks (e.g. blurry image, RS image, keyframe pair, etc. with corresponding events), and setting the neural shutter to a randomly chosen ground truth, specifically, we can set $t_a(x,y)=t_b(x,y)=t_{gt}$ where $t_{gt}$ can be arbitrary timestamp of a sharp GS image, and we can set the neural shutter identical to the timestamp of input real-captured image to force the model perform reconstruction.
% Specifically, the input of the network can be one or two real-captured frames which are sharp or blurry, global shutter or rolling shutter images,
% and the neural shutter is randomly set to the shutter strategy of a ground truth image, and the resulted target image will be compared with the ground truth.
Both training strategies are conducted in the supervised way, where we adopt a combination of a Charbonnier loss~\cite{CharbonnierLoss}, a perceptual loss~\cite{PerceptualLoss}, and a PSNR loss~\cite{HINet} as the target function. 
We randomly crop the input into $256\times256$ patches in training. We train our model with 60000 iterations with a batch size of 32 on a Tesla A100 GPU.


\begin{table}[h!]
	% 多任务训练与单任务训练的对比
	\centering
	\caption{Comparison of specialized and versatile NIRE (in PSNR/SSIM)}
	\resizebox{1.0\columnwidth}{!}{
	\begin{tabular}{c|cccc}
		\toprule
		\diagbox{task}{strategy}& MT          & VFI         & Deblur      & Unroll      \\
		\hline
		VFI           & 34.97/0.964 & 34.44/0.955 & -           & -           \\
		Deblur        & 35.03/0.973 & -           & 34.72/0.966 & -           \\
		Unroll        & 30.08/0.909 & -           & -           & 30.04/0.909 \\
		Deblur+Unroll & 29.86/0.908 & -           & -           & -           \\
		Deblur+VFI    & 33.43/0.948 & -           & -           & -        \\
		\bottomrule  
	\end{tabular}
	\label{tab:spec-vs-vers}
	}
\end{table}

We compare the two training strategies on different tasks. As shown in tab.~\ref{tab:spec-vs-vers} the models trained with the first strategies (VFI, Deblur, Unroll) can only perform their specialized tasks
while the model trained with the second strategy (MT) is able to handle all tasks simultaneously with better or comparable performance.
Additionally, when there are multiple issues for the real-captured frames (e.g. Deblur+Unroll, Deblur+VFI), 
the proposed method is still competent, making it a more practical method for frame restoration.

As we purpose to develop a versatile frame restoration method, we adopt the multi-task training strategy in the following experiments by default.

\subsection{Datasets}
% Introduce dataset
We use two datasets, GoPro~\cite{GoProDataset} and Gev-RS~\cite{EvUnroll}, for training and quantitative evaluation in our experiments. 
GoPro~\cite{GoProDataset} is a dataset consisting of sequences shot by a GoPro camera with a frame rate of 240 FPS and a resolution of 1280$\times$720, 
providing training samples and evaluation benchmarks for tasks including deblurring, frame interpolation, and jointly deblurring and frame interpolation.
Gev-RS~\cite{EvUnroll} is a dataset developed for event-base rolling shutter correction with sequences of 5700 FPS frames for high quality event simulation. Gev-RS provides training samples and evaluation benchmarks for the unrolling task in our experiment.
In addition, Zhou \etal~\cite{EvUnroll} collect some real-captured RS-event pairs, which we adopt for qualitative unrolling evaluation. And we collect some real blurry-event pairs for qualitative deblurring evaluation.
For each task, we follow the common practice of evaluation to achieve fair comparison.

\subsection{Deblur}
Following the deblurring practice~\cite{GoProDataset}, the GoPro dataset is arranged into 3214 blurry-sharp image pairs, in which there are 2103 pairs for training and 1111 pairs for testing. 
The blurred images are produced by averaging several consecutive sharp frames.
And following the practice of event-based deblurring~\cite{EDI}~\cite{EFNet},
we use an event camera simulator~\cite{V2E-Simulator} to obtain frame-aligned event data.

\begin{table}[h!]
\centering
\caption{\textbf{Performance on deblurring}}
\resizebox{0.75\columnwidth}{!}{
\begin{tabular}{@{}lcccc@{}}
	\toprule
	\textbf{Methods}  			&\textbf{event} & \textbf{arbitary}	& \textbf{PSNR} & \textbf{SSIM} \\
	\midrule
	E2VID~\cite{E2VID} 			&\ding{51}		&\ding{51}			& 15.22         & 0.651  	    \\
	DeblurGAN~\cite{DeblurGAN}	&\ding{55}		&\ding{55}			& 28.70         & 0.858         \\
	EDI~\cite{EDI}     			&\ding{51}		&\ding{55}			& 29.06         & 0.940         \\
	DeepDeblur~\cite{DeepDeblur}&\ding{55}		&\ding{55}			& 29.08         & 0.914         \\
	DeblurGAN-v2~\cite{Dbl-v2}	&\ding{55}		&\ding{55}			& 29.55         & 0.934         \\
	SRN~\cite{SRN}     			&\ding{55}		&\ding{55}			& 30.26         & 0.934         \\
	SRN+~\cite{SRN}   			&\ding{51}		&\ding{55}			& 31.02         & 0.936         \\
	DMPHN~\cite{DMPHN}          &\ding{55}		&\ding{55}		    & 31.20         & 0.940         \\
	D$^2$Nets~\cite{D2Net}		&\ding{51}		&\ding{55}			& 31.60         & 0.940         \\
	LEMD~\cite{LEMD}		    &\ding{51}		&\ding{55}			& 31.79         & 0.949         \\
	Suin et al.~\cite{SAPHNet}	&\ding{55}		&\ding{55}			& 31.85         & 0.948         \\
	SPAIR~\cite{SPAIR} 			&\ding{55}		&\ding{55}			& 32.06         & 0.953         \\
	MPRNet~\cite{MPRNet}		&\ding{55}		&\ding{55}			& 32.66         & 0.959         \\
	HINet~\cite{HINet} 			&\ding{55}		&\ding{55}			& 32.71         & 0.959         \\
	ERDNet~\cite{ERDNet}		&\ding{51}		&\ding{55}			& 32.99         & 0.935         \\
	HINet+~\cite{HINet}			&\ding{51}		&\ding{55}			& 33.69         & 0.961         \\
	EFNet~\cite{EFNet} 			&\ding{51}		&\ding{55}			& \textbf{35.46} 		& 0.972         \\
	\midrule
	NIRE 						&\ding{51}		&\ding{51}			& 35.03         & \textbf{0.973}         \\

	\bottomrule
\end{tabular}
}
\label{tab:prec_deblur}
\end{table}

As shown in tab.~\ref{tab:prec_deblur},
the NIRE outperforms the conventional frame-based deblur method,
and achieves comparable performance with the state-of-the-art event-based method,
demonstrating that NIRE is competent for deblurring task.
Interestingly, as opposed to existing methods that typically restore the sharp frame of a fixed instant (e.g. the mid instant of exposure),
the proposed method is able to produce images of arbitrarily specified instants, 
even unfolding a blurry image into a clip of a video with an extremely high frame rate. \xinyu{including unfolding demo in supp?}


\subsection{Video Frame Interpolation}
To verify the effectiveness of our method on frame interpolation task,
we evaluate NIRE following the practical setting of event-based frame interpolation\cite{TimeLens} on GoPro. 
As shown in tab.~\ref{tab:prec_vfi_gopro}, NIRE achieves much better performance than the conventional frame-based methods,
and slightly surpasses the event-based TimeLens~\cite{TimeLens} method on 7-skip settings.
On 15-skip settings, NIRE achieves slightly lower performance than TimeLens, 
indicating the construction of long-range visual latent space remains to be improved.
\begin{table}[h!]
\caption{\textbf{Performance on video frame interpolation}}
\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{lccllll}
	\toprule
	\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multirow{2}{*}{\textbf{frames}} & \multirow{2}{*}{\textbf{events}} & \multicolumn{2}{l}{\textbf{7 frames skip}}
	& \multicolumn{2}{l}{\textbf{15 frames skip}} \\ \cmidrule(l){4-7} 
	
	\multicolumn{1}{c}{} 	& 			& 			& PSNR  & SSIM  & PSNR  & SSIM   \\ 
	\midrule
	DAIN~\cite{DAIN}		&\ding{51} 	&\ding{55}	& 28.81 & 0.876 & 24.39 & 0.736  \\
	SuperSloMo~\cite{SloMo}	&\ding{51} 	&\ding{55}	& 28.98 & 0.875 & 24.38 & 0.747  \\
	RRIN~\cite{RRIN}		&\ding{51} 	&\ding{55}	& 28.96 & 0.876 & 24.32 & 0.749  \\
	BMBC~\cite{BMBC}		&\ding{51} 	&\ding{55}	& 29.08 & 0.875 & 23.68 & 0.736  \\
	E2VID~\cite{E2VID}		&\ding{55} 	&\ding{51} 	& 9.74  & 0.549 & 9.75  & 0.549  \\
	EDI~\cite{EDI}			&\ding{51} 	&\ding{51} 	& 18.79 & 0.670 & 17.45 & 0.603  \\
	% TimeReplayer~\cite{TimeLens}&\ding{51} 	&\ding{51} 	& 34.02 & 0.960 & - & -  \\
	TimeLens~\cite{TimeLens}&\ding{51} 	&\ding{51} 	& 34.81 & 0.959 & 33.21 & 0.942  \\
	\midrule
	NIRE-vfi 		&\ding{51} &\ding{51} 	& 34.97 & 0.964 & 32.85 & 0.945  \\	
	\bottomrule
\end{tabular}
}
\label{tab:prec_vfi_gopro}
\end{table}


\subsection{Rolling Shutter Correction}

%The key that NIRE is able to correct the rolling shutter effect is that it is capable of constructing the visual latent space from RS (rolling shutter) images.
Different from GS (global shutter) images, pixels in an RS image start and end exposing at different instants,
containing information of varying temporal ranges.
Benefiting from the time encoding, NIRE can identify this variation, 
adaptively arranging the information of each pixel into the visual latent space.
And by defining the neural shutter of every pixel to the same instant, the produced image will be free of rolling shutter effect.

\begin{table}[h!]
	\centering
	% \caption{\textbf{Performance of rolling shutter correction on Gev-RS~\cite{EvUnroll} dataset}. * indicates the version without time encoding for RS image}
	\caption{\textbf{Performance of rolling shutter correction on Gev-RS~\cite{EvUnroll} dataset}.}
	\resizebox{0.7\columnwidth}{!}{
		\begin{tabular}{lccc}
			\toprule
			\textbf{Methods}  	& \textbf{events} 	& \textbf{PSNR}  	& \textbf{SSIM} \\	% & \textbf{LPIPS} \\
			\midrule
			DSUN~\cite{DSUN}	& \ding{55}	  		& 23.10 			& 0.70 \\ 				% & 0.166 \\
			JCD~\cite{JCD}      & \ding{55}	  		& 24.90 			& 0.82 \\				% & 0.105 \\
			EvUnroll~\cite{EvUnroll}& \ding{51}     & 30.14 			& 0.91 \\				% & 0.061 \\
			\midrule
			% NIRE*			& \ding{51}      	& 27.34 				& 0.86 \\				% & 0.081 \\  % without time encoding corresponding to RS image
			% NIRE     			& \ding{51}      	& 30.05 			& 0.91  \\ 			% & 0.063 \\  % historical best result, may caused by randomness
			NIRE     			& \ding{51}      	& 29.86 			& 0.91 \\				% & 0.065 \\
			\bottomrule
		\end{tabular}
	}
	\label{tab:prec_unroll_gevrs}
\end{table}

As shown in tab.~\ref{tab:prec_unroll_gevrs},
the method outperforms the frame-based methods and achieves comparable performance with the state-of-the-art event-based method EvUnroll~\cite{EvUnroll},
demonstrating NIRE is capable of constructing the visual latent space from an RS image.
% And it can be observed that excluding the time encodings of the visual latent space significantly impairs the performance, 
% implying the importance of time encodings for processing rolling shutter images.  
It is worth noting that the Gev-RS benchmark implicitly involves the task of deblurring because the RS frames as input in this dataset are blurry and the ground truths are sharp.
Hence the competitive performance also indicates NIRE can jointly address rolling shutter effect and motion blur without cascading or other specially designed architecture.

Zhou \etal~\cite{EvUnroll} provides some real-captured data for qualitative evaluation. As shown in fig.~\ref{fig:qualitative-real}, the proposed method works normally on real-captured data. It is worth noting there is no ground truth available for finetuning on the real-captured data.

% \begin{figure}[h!]
% 	\centering
% 	\includegraphics[width=1.0\columnwidth]{figs/qualitative-real.pdf}
% 	\caption{Qualitative result on real-captured data for unrolling.}
% 	\label{fig:qualitative-real}
% 	\vspace{-1.0em}
% \end{figure}

\begin{figure}[h!]
	\centering
	\includegraphics[width=1.0\columnwidth]{figs/qualitative-real2.pdf}
	\caption{Qualitative result on real-captured data without finetuning. More results are available in supplementary material.}
	\label{fig:qualitative-real}
	\vspace{-1.0em}
\end{figure}

\subsection{Joint Deblur and Frame Interpolation}

Typically, video frame interpolation presumes the key frames are sharp, 
especially for the warping-based methods.
However, it is common that the key frames are affected by motion blur, 
which subsequently impacts the quality of the interpolated frames.
An intuitive solution is to cascade a deblurring model and a VFI model.
But simply cascading two models will lead to error accumulation and domain gap, 
which subsequently reduces the performance.

\begin{table}[h!]
\centering
\caption{\textbf{Performance on Joint Deblur and Frame Interpolation}}
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{@{}lllll@{}}
	\toprule
	\textbf{Methods}          	& \textbf{unified}  & \textbf{events}   & \textbf{PSNR}  & \textbf{SSIM}   \\
	\midrule
	% BIN: https://arxiv.org/pdf/2002.12259.pdf - without data on GoPro
	% 
	SRN~\cite{SRN} + SloMo~\cite{SloMo}      &\ding{55}		&\ding{55} 			& 24.72 & 0.7604 \\  % https://sci-hub.hkvisa.net/10.1109/tip.2020.3033617
	SRN + MEMC-Net~\cite{MEMC-Net}     		&\ding{55}		&\ding{55} 			& 25.70 & 0.7792 \\  % https://sci-hub.hkvisa.net/10.1109/tip.2020.3033617
	SRN + DAIN~\cite{DAIN}       			&\ding{55}		&\ding{55} 			& 25.17 & 0.7708 \\  % https://sci-hub.hkvisa.net/10.1109/tip.2020.3033617
%	EDVR + QVI       			&\ding{55}		&\ding{55} 			& 28.57 & 0.9152 \\  % https://arxiv.org/pdf/2112.01161.pdf
%	EDVR + SloMo     			&\ding{55}		&\ding{55} 			& 27.74 & 0.9010 \\  % https://arxiv.org/pdf/2112.01161.pdf
	EDVR~\cite{EDVR} + SloMo	&\ding{55}		&\ding{55} 			& 24.85 & 0.7762 \\  % https://sci-hub.hkvisa.net/10.1109/tip.2020.3033617
	EDVR + MEMC-Net    			&\ding{55}		&\ding{55} 			& 27.12 & 0.8301 \\  % https://sci-hub.hkvisa.net/10.1109/tip.2020.3033617
	EDVR + DAIN      			&\ding{55}		&\ding{55} 			& 29.01 & 0.8981 \\  % https://sci-hub.hkvisa.net/10.1109/tip.2020.3033617
%	UTI-VFI          			&\ding{51}		&\ding{55} 			& 25.63 & 0.8148 \\	 % https://www.ecva.net/papers/eccv_2022/papers_ECCV/papers/136670193.pdf
	UTI-VFI~\cite{UTI-VFI}		&\ding{51}		&\ding{55} 			& 29.73 & 0.8873 \\  % https://www.ecva.net/papers/eccv_2022/papers_ECCV/papers/136670193.pdf
	TNTT~\cite{TNTT}   			&\ding{51}		&\ding{55} 			& 26.68 & 0.8148 \\  % https://www.ecva.net/papers/eccv_2022/papers_ECCV/papers/136670193.pdf
	PRF~\cite{PRF}     			&\ding{51}		&\ding{55} 			& 25.68 & 0.8053 \\  % https://www.ecva.net/papers/eccv_2022/papers_ECCV/papers/136670193.pdf
	DeMFI-Net~\cite{DeMFI}		&\ding{51}		&\ding{55} 			& 31.25 & 0.9102 \\  % https://www.ecva.net/papers/eccv_2022/papers_ECCV/papers/136670193.pdf
	\midrule
	NIRE-dbl+vfi     			&\ding{55}		&\ding{51} 			& 30.18 & 0.8923 \\
	NIRE		       			&\ding{51}		&\ding{51} 			& 33.43 & 0.9477 \\
	\bottomrule
\end{tabular}
\label{tab:prec_jdfi_gopro}
}
\end{table}

Fortunately, NIRE is naturally capable of jointly addressing motion blur and discontinuity.

Following Oh et al.~\cite{DeMFI}, we re-arrange the GoPro dataset to train and evaluate the performance on joint deblurring and frame interpolation.
As shown in tab.~\ref{tab:prec_jdfi_gopro}, NIRE surpasses existing methods by a large margin, 
demonstrating its advantage in jointly addressing motion blur and video discontinuity.
We also try to address deblur and frame Interpolation sequentially by using NIRE twice (NIRE-dbl+vfi), 
which achieves significantly worse performance than addressing them in a unified manner,
demonstrating the advantage of end-to-end unification.
\xinyu{TODO: don't konw where to introduce Fig.~\ref{fig:qualitative_results}}


\subsection{Ablation}

We perform an ablation study to find out the necessity of components. 

\begin{table}[h!]
\caption{\textbf{Ablation Study}}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{ccccc}
\toprule
Tasks     & VFI         & Deblur      & Unroll      & Deblur+VFI  \\ 
\hline
NIRE    & 34.97/0.964 & 35.03/0.973 & 29.86/0.908 & 33.43/0.948 \\
% w/o Time Encoding & 31.23/0.921 & 33.44/0.955 & 20.38/0.584 & 29.76/0.874 \\
w/o Event & 30.40/0.886 & 29.53/0.928 & 24.08/0.803 & 26.46/0.815 \\
w/o FeatEnhance   & 32.83/0.928 & 33.78/0.952 & 26.42/0.835 & 30.62/0.894 \\ 
\bottomrule
\end{tabular}}
\label{tab:ablation}
\end{table}

As shown in tab.~\ref{tab:ablation}, excluding any timer, event feature, or feature enhancement from our model lead to significant drop of performance.
Without the timer\footnote{Only the timer for neural shutter is kept}, the model will have no idea about the temporal relationship between the frames and events, leading to potential misalignment of the two sources, especially for the unrolling task. 
The event is the important source of the visual latent space. Without event, the information for visual latent space is incomplete. The inter-attention layer is the module for expanding the receptive filed. Without inter-action layers, the model will fail to aggregate long range information, especially when the objects in the scene have large displacement. 



==> sections/2_related_works_v1.tex <==


\section{Related Works}

% \subsection{Video Restoration}
%
% Existing methods tend to address these issues from the perspective of their specific causes and characteristics.
% For example, algorithms for frame interpolation~\cite{bibid} typically estimate the motion field of the frames to predict the trajectory of each pixel.
% To restore the motion blur, deblurring algorithms~\cite{bibid} may establish the motion model that causes blurring, 
% restoring the confused temporal information with an implicitly or explicitly estimated the blurring kernel, 
% or collecting information from adjacent frames as an extra clue.
% For rolling shutter correction, 
% algorithms~\cite{bibid} typically evaluate the velocity of each pixel, then infer and reverse the displacement of them to restore the temporal misalignment.
% Although these methods are effective, they are limited to their specialized domains.

% % 介绍我们的思路：我们通过类比exposure，整合了三个任务。
% Instead of delving into specific causes or characteristics, 
% we propose to establish a model simulating the process of exposure to restore arbitrary expected frames.


\subsection{Motion Deblur}
Motion blur often occurs when the object or camera moves at high speed during exposure time. Some methods~\cite{kernel1,kernel2} model blurry image and sharp image with blur kernel and deblur images with deconvolution network, which is difficult to deal with spatial inconsistent blur. Recently, some methods~\cite{DeepDeblur,MIMO,NAFNet} build architecture based on U-Net~\cite{U-Net} to deblur images in coarse-to-fine strategy. However, due to the complexity of blur patterns and the lack of temporal information during exposure time, the effect is still limited when facing complex motion scenes.

There is rich temporal information with events triggered during exposure period, which is very helpful in removing motion blur in the image. Pan \etal~\cite{EDI} first proposed the Event-based Double Integral (EDI) model to model the event, blurry image and sharp image, which outputs sharp image by optimizing the energy function. Considering the impact of noise and the unknown threshold of events, some methods ~\cite{LEMD,LEDVDI,EVDI} use deep learning networks to calculate the sharp image based on the same principle. According to the study of the relationship between image gradient and events, Song \etal~\cite{E-CIR} try to represent a video by per-pixel parametric polynomials using a deep learning model. Xu \etal~\cite{REDNet} use the event to predict optical flow to supervise the output images while deblurring. By studying the impact of light on event noise, Zhou \etal~\cite{lowlight} attempt to estimate the blur kernel with event, and then deblur images by deconvolution. Sun \etal~\cite{EFNet} proposed a cross-modal channel-wise attention module to fuse event features and image features at multiple levels.

\subsection{Video Frame Interpolation}
Because of lack of motion information between frames, most RGB-only frame interpolation methods~\cite{SloMo,AdaCoF,DAIN,RIFE} are based on linear motion assumption. These methods calculate the optical flow according to the difference between two images, linearly calculate the optical flow from input timestamp to output timestamp and finally warp image with the optical flow. 

Compared with RGB interpolation, multi-modality interpolation methods are more robust due to the rich motion information of event, which makes it applied to complex motion scene. Zhang \etal~\cite{EVDI} proposed a fully self-supervised and unified framework of deblur and interpolation. Xu \etal~\cite{REDNet} try to predict optical flow between output frames to simulate nonlinear motion during exposure time. He \etal~\cite{timereplay} proposed a unsupervised method that the output image can be predicted according to the input image while the input image can be predicted by input graph in turn. Tulyakov \etal~\cite{TimeLens} design a warping based module and a systhesis based module to fully extract motion clue and photometric change information from event. 

\subsection{Rolling Shutter Correction}
Rolling shutter effect caused by the fact that the image is captured in a progressive scan, meaning that each row of pixels is exposed at a different time. Similar to frame interpolation, RGB-based unrolling task mostly depends on the optical flow and linear motion assumption. Referring to ~\cite{SloMo} structure, Fan \etal~\cite{RSSR,CVR} firstly proposed to calculate the optical flow between two input rolling shutter images, and then predict global shutter image according to the optical flow. Fan \etal~\cite{SUNet} and Liu \etal~\cite{DSUN} use pyramidal construction, calculate the cost volume at the feature level to get motion clue which is used to warp the feature or image to get final global shutter image. Zhou \etal~\cite{EvUnroll} design a two-branch structure to solve the generic rolling shutter correction problem with two consecutive frames.

\subsection{Joint Task}
There have already been some efforts~\cite{EVDI, EvUnroll, LEDVDI, DeMFI} in dealing with multiple tasks at the same time. Oh \etal~\cite{DeMFI} take only four blurry images as input which consists of a flow-guided module for deblurring and a recursive boosting module for interpolation. Zhang \etal~\cite{EVDI} first process two continuous blurry images and corresponding events separately to predict sharp images at the same timestamp, and then fuse two sharp images with weights which related to time interval between sharp image and blurry images. Simply, it deblurs images in stage one and fuse images in stage two. Lin \etal~\cite{LEDVDI} propose an end-to-end trainable neural network to utilize the physical information of the event. It firstly deblurs frames according to EDI~\cite{EVDI} model same as other event deblurring methods, and secondly interpolates frames with sharp image predicted before and the event which indicates the brightness change. Zhou \etal~\cite{EvUnroll} deblur and unroll images with event in a two-branch structure. But the deblurring module is optional which means it's independent of unrolling task.

However, most works address multiple tasks with separate modules in , but not in a unified framework.
Compared to the methods mentioned above which only addressing one or two specialized issues, our method propose a unified framework to deal with all these shutter-related problems. 






% \subsection{Time aware feature}
% Visual latent space uses time encoding.

% \subsection{Simulated Camera}
% \cite{Ouyang_Neural_Camera_Simulators}

% As opposed to neural representation that implicitly models the 3D structure of the scene, 
% the proposed neural camera only models the content captured by the lens.

%Rolling shutter correction is the process of correcting distortions in images or videos that have been captured using a rolling shutter camera. A rolling shutter camera captures an image or video by scanning the scene line by line, rather than capturing the entire image or video all at once. This can result in distortions in the captured image or video, such as skew, wobble, and bend, due to the motion of the camera or the objects in the scene during the scanning process.

\begin{figure}[t]  % figure of 3d block
	\centering
	\includegraphics[width=0.9\columnwidth]{figs/fig_01.pdf}
	\caption{
		Sensor data from which the visual latent space is constructed.
		The real-captured frames are presented as 3-D blocks, from left to right are a sharp GS frame, a blurry GS frame, a sharp RS frame, a blurry RS frame, and another sharp GS frame.
		 Each Encapsulate a sub-domain of the visual content, 
		while the events fill the whole spatial-temporal space.
		Complementing each other, 
		they provide abundant information for constructing a comprehensive visual latent space.
		%Illustration of the materials for optical content reconstruction.
		%From left to right, the sharp GS frame, blurry GS frame, sharp RS frame, blurry RS frame, and another sharp GS frame are presented as 3-D blocks.
		%Intuitively, the thicker the shutter blocks, the more blurry the images will be.
		%Events fill the whole spatial-temporal domain, complementing vacant part left by the images.
		%For intuitive comprehension, we conduct some visualizations in fig.~\ref{fig:sensor_data}.
		%The coordinate denotes the spatial-temporal domain where $\Omega(x, y; t)$ is defined.
		%The open periods of the shutter are visualized as some blocks called ``shutter blocks".
		%It can be observed that the blocks for different shutter mechanisms take on different shapes.
		%% 每个shutter block包含了$\Omega(x, y; t)$的一个子域，表明图片是对optical content的一种采样
		%Each shutter block encapsulates a subdomain of $\Omega(x, y; t)$, 
		%suggesting the images are actually samples of optical content.
	}
	\label{fig:sensor_data}
	\vspace{-1.0em}
\end{figure}

